DeepRec: Towards a Deep Dive Into the Item Space with Large Language Model Based Recommendation

Recently, large language models (LLMs) have been introduced into recommender systems (RSs), either to enhance traditional recommendation models (TRMs) or serve as recommendation backbones. However, existing LLM-based RSs often do not fully exploit the complementary advantages of LLMs (e.g., world knowledge and reasoning) and TRMs (e.g., recommendation-specific knowledge and efficiency) to fully explore the item space. To address this, we propose DeepRec, a novel LLM-based RS that enables autonomous multi-turn interactions between LLMs and TRMs for deep exploration of the item space. In each interaction turn, LLMs reason over user preferences and interact with TRMs to retrieve candidate items. After multi-turn interactions, LLMs rank the retrieved items to generate the final recommendations. We adopt reinforcement learning(RL) based optimization and propose novel designs from three aspects: recommendation model based data rollout, recommendation-oriented hierarchical rewards, and a two-stage RL training strategy. For data rollout, we introduce a preference-aware TRM, with which LLMs interact to construct trajectory data. For rewards, we design a hierarchical reward function that involves both process-level and outcome-level rewards to optimize the interaction process and recommendation performance, respectively. For RL training, we develop a two-stage training strategy, where the first stage aims to guide LLMs to interact with TRMs and the second stage focuses on performance improvement. Experiments on public datasets demonstrate that DeepRec significantly outperforms both traditional and LLM-based baselines, offering a new paradigm for deep exploration in recommendation systems.

==> sec_preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}

In this section, we first formulate the sequential recommendation task and then describe existing LLM-based recommendation systems for the task.

\paratitle{Task Formulation.}
Sequential recommendation~(SR) aims to capture the user's dynamic preferences from his/her historical behaviors and predict the next potential item.
Formally, given the item set $\mathcal{V}$, a user’s historical interactions are represented as an item sequence $S_n = [v_1, \dots, v_n]$ in chronological order.
The recommendation task can be formulated as $P(v_{n+1}|S_n)$, that is, next item prediction based on user historical interactions.

\paratitle{LLM-based Recommendation Systems.}
Existing LLM-based recommendation systems~(RSs) for SR can be divided into three main categories according to the relationship between LLMs and traditional recommendation models~(TRMs).

$\bullet$~\textit{LLM-enhanced TRM.}
This approach utilizes TRMs to make the recommendation and introduces LLMs as auxiliary components to help TRMs~\cite{}.
Since TRMs are trained only on observed user interaction data, they do not have enough factual knowledge about each interacted item.
In contrast, LLMs are trained on massive textual corpora with abundant world knowledge.
Therefore, LLMs can provide extra features about items or augment user interaction data for TRMs.
Formally, TRMs accept user interaction history $S_n$ and augmented features or data $A_n$ from LLMs as the input to predict the next item $v_{n+1}$, which can be represented as follows:
\begin{equation}
    \text{Pr}(v_{n+1} | S_n) = \text{Pr}_{\text{TRM}}(v_{n+1} | S_n, A_n) \cdot \text{Pr}_{\text{LLM}}(A_n | S_n)
\end{equation}
% However, this approach often suffers from misalignment, as general LLMs are not specially optimized for SR.
% In addition, it fails to leverage the reasoning capability of LLMs for SR. 

$\bullet$~\textit{TRM-enhanced LLM.}
Different from LLM-enhanced TRM, this approach utilizes LLMs to make the final recommendation and introduces TRMs as auxiliary components~\cite{}.
Since LLMs excel at complex reasoning and TRMs specialize in efficient matching, the common practice is to first use TRMs to retrieve a subset of candidate items and then use LLMs to rank these candidates for recommendation.
Formally, LLMs accept user interaction history $S_n$ and retrieved items $I_n$ from TRMs as the input to predict the next item $v_{n+1}$, which can be represented as follows:
\begin{equation}
    \text{Pr}(v_{n+1} | S_n) = \text{Pr}_{\text{LLM}}(v_{n+1} | S_n, I_n) \cdot \text{Pr}_{\text{TRM}}(I_n | S_n)
\end{equation}
% As an alternative form of LLM-based recommendation, some methods employ a traditional recommender to pre-retrieve candidate items before applying LLM for final recommendation. 
% Unlike straightforward recommendation, this approach does not require the LLM to explore potential items from the entire item pool.
% Consequently, the textual item title can be directly used to represent the item, which is conducive to the adaptation of the LLM to recommender systems.
% Formally, given the candidate items $O$ pre-retrieved by the traditional recommender, it is concatenated with the user's historical behaviors $X$ as input. Then, the LLM generates the target item or recommendation list $Y$:
% \begin{align}
% P(Y|X)= P_{\text{\scriptsize LLM}}(Y|X,O)) \cdot P_{\text{\scriptsize Rec}}(O|X)),
% \end{align}
% where $P_{\text{\scriptsize Rec}}(\cdot)$ denotes the probability function of the traditional recommender.

$\bullet$~\textit{LLM as RS.}
Different from the above two approaches, it uses LLMs for end-to-end recommendation.
To ensure the validity of generation, this approach typically introduces concise and standardized item identifiers (\eg semantic IDs~\cite{}) into the vocabulary of LLMs and utilizes several tokens to represent one item.
Formally, LLMs accept user interaction history $S_n$ as the input to directly predict the identifier of the next item $v_{n+1}$, which can be represented as follows:
\begin{equation}
    \text{Pr}(v_{n+1} | S_n) = \prod_{i=1}^{|v_{n+1}|} \text{Pr}_{\text{LLM}}(v_{n+1}^i | S_n, v_{n+1}^{<i}),
\end{equation}
where $v_{n+1}^i$ is the $i$-th token of $v_{n+1}$ and $v_{n+1}^{<i}$ is the tokens preceding the $i$-th position.

% In order to make item generation easier and ensure the generation of valid items, this paradigm typically introduces concise and standardized item identifiers (\eg semantic IDs~\cite{}) into LLM vocabulary, and trains the model to directly generate the target item identifiers.
% Specifically, the user's historical interactions $s$ are represented as a token sequence by concatenating item identifiers. 
% Then, this sequence is combined with the recommendation task description into an instruction $X$. 
% Finally, $X$ is fed into LLMs to autoregressively generate the target item identifier $Y$.
% Formally, the task can be written as:
% \begin{align}
% P(Y|X)=\prod_{j=1}^{|Y|}P_{\text{\scriptsize LLM}}(Y_i|X,Y_{<i}),
% \end{align}
% where $Y_i$ is the $i$-th token of $Y$, and $Y_{<j}$ represents the token before $Y_i$. $P_{\text{\scriptsize LLM}}(\cdot)$ is the probability function of LLM.
% This paradigm allows LLMs to freely explore potential items from the global environment and the entire item pool, but it also amplifies the requirement for domain-specific knowledge in the recommendation scenarios.
